SmartCert: Redesigning Digital Certificates with Smart Contracts

The Transport Layer Security (TLS) protocol and its public-key infrastructure (PKI) are widely used in the Internet to achieve secure communication. Validating domain ownership by trusted certification authorities (CAs) is a critical step in issuing digital certificates, but unfortunately, this process provides a poor security level. In this work, we present SmartCert, a novel approach based on smart contracts to improve digital certificates. A certificate in SmartCert conveys detailed information about its validation state which is constantly changing but only with respect to the specified smart contract code and individual domain policies. CAs issuing and updating certificates are kept accountable and their actions are transparent and monitored by the code. We present the implementation and evaluation of SmartCert, and discuss its deployability.

==> sec_app_eval.tex <==
\myparagraph{Smart Contracts}
  Deploying and interacting with
smart contracts over Ethereum is associated with a gas cost.  Each operation
costs a pre-defined amount of gas, and operations can differ significantly in
their gas consumption.  To estimate the cost in US dollars we used the following
data from \url{https://ethgasstation.info/} obtained on 20 Jan 2019: we used the
\textit{standard gas price} equal 2.15 Gwei/gas (1 Gwei = $10^{-9}$ ether) with the
ether price equal \$125/ether.  Due to the high volatility of ether prices, we
emphasize that the presented cost in USD is only an estimation.
We deployed our smart contracts on an Ethereum testnet.

First, we measured the cost incurred by registering a policy with the policy
contract (see \textit{newPolicy()} in \autoref{alg:policy}).  The overall cost
obtained is 867034 gas, which in our setting translates to \$0.23. This cost is
mainly due to the transaction size and the storage required to store the policy
fields. Authentication of policies by additional CAs is relatively cheap, as a single
signature verification costs only 3000 gas.  

Next, we investigated how expensive it is to deploy \name certificates.  In our
experiment, the contract was deployed for the \url{facebook.com} domain, with
which a CA kept conducting TLS handshakes periodically (with client random
values set to recent block hashes) and kept submitting obtained validation
proofs to update the \name contract.  \url{Facebook.com} signs ServerKeyExchange
messages with RSA-2048 and the results of this experiment are presented in
\autoref{tab:cost}.  As shown in the table, creating the contract and
initializing its storage is more expensive than updating it, and according to
our estimation, it costs around \$0.36. This is, however, a one-time operation
per \name contract.  To update a \name contract by a validation proof, a CA has
to pay about \$0.05 in that scenario.  As depicted, the RSA verification is the
\textit{update()}'s dominant operation, consuming almost 56\% of all gas
required.

\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{|c||r|r|r|r|}
    \cline{3-5}
    \multicolumn{1}{c}{} &
    \textbf{create}&\multicolumn{3}{|c|}{\textbf{\textit{update()}}} \\
    \cline{3-5}
    \multicolumn{1}{c}{} &
    \textit{\textbf{+ init()}} & \textbf{Total } &
    $\textbf{\textit{SigVrfy()}}$ & \textbf{Misc.\ \ }\\
    \hline
    \hline
    Gas&1343799&165885&92623&73261\\
    ETH&0.00289&0.00036&0.0002&0.00016\\
    USD&\$0.361&\$0.045&\$0.025&\$0.020\\
    \%&100\%&100\%&55.8\%&44.2\%\\
    \hline
    % \hline
    % \multirow{4}{*}{RSA-1024}&Gas&1254803&103144&46107&57037\\
    % % \cline{2-6}
    % &ETH&0.0027&0.0002&0.0001&0.0001\\
    % &USD&\$0.337&\$0.028&\$0.012&\$0.015\\
    % &\%&100\%&100\%&44.8\%&55.3\%\\
    % \hline
\end{tabular}
\caption{Cost analysis of the \name contract operations.}
\label{tab:cost}
\end{center}
    \vspace{-0.3cm}
\end{table}

% For comparison, we investigated the same operations but using RSA-1024
% signatures (although this key length is not recommended, it is still
% popular~\cite{ssllabs}).  In this setting, creating and initializing a \name
% contract costs about \$0.34.  The price difference is mainly due to the
% difference between the lengths of public keys that the contract has to store.
% An execution of \textit{update()} is less costly too, requiring about \$0.03 per
% update.  In that case, the signature
% verification still incurrs a significant cost -- around 45\% of
% the total update cost.

The cost of maintaining a \name certificate over the Ethereum blockchain is
mainly determined by the epoch parameter, which we discuss  in detail in
\autoref{pre:practical:params}. In \autoref{tab:month} we present a monthly
cost depending on potential epoch values assuming a single CA (the cost is
linear to the number of CAs).  As shown, the cost is inversely proportional to
the epoch, and e.g., the monthly cost for a \name certificate validated every
day is around \$1.25.

\begin{table}[t]
    % \vspace{-0.75cm}
\begin{center}
    \small
    \begin{tabular}{c|rrrrr}
        \textbf{Epoch}    & 6h  &   12h   &   24h  &  48h &  72h  \\ \hline
        \textbf{Cost}     & \$5.05  &\$2.53 & \$1.26 &\$0.63 & \$0.42 \\
    \end{tabular}
    \caption{A monthly deployment cost depending on epoch values.}
    \label{tab:month}
    \end{center}
    \vspace{-0.3cm}
\end{table}


Ethereum, like other blockchain platforms, is under heavy development.
Therefore, we envision that with scaling solutions and more mature
implementations (e.g., natively-supported RSA operations), the gas consumption
presented may be much lower in future, consequently lowering the overall cost of
\name deployment.
% \medskip


\myparagraph{CAs} 
The main overhead on the CA's side is to conduct periodic validations. This
process does not require any new protocol as CAs just run TLS handshakes (as
presented in \autoref{sec:details:valid}).  In order to estimate the throughput, we conducted an
experiment.  We selected random 10000 Internet hosts supporting TLS and we
conducted periodic TLS handshakes with them.  We used a machine equipped with
Intel Core i7 (3.5GHz), 16GB RAM, and connected to the Internet via a 100Mbps
wired link.  This single machine running connections in parallel could perform
around 175 TLS handshakes per second on average, i.e., 0.63M handshakes per
hour. % (this time is dominated by the network latency). Therefore, assuming epoch
% equal six hours, a few machines could validate a number of public keys
% similar to the number of active TLS certificates currently issued by even large
% CAs~\cite{vandersloot2016towards,ca_usage}.


\myparagraph{Transmission Overhead}
Size of a \name certificate is the only transmission overhead introduced to a
\name-enabled TLS connection. In order to estimate it, we used a \name
certificate derived from the \name contract deployed in the previous experiment.
The main contributors to the \name certificate size are MPT storage and code 
proofs ($\pi_{s}$ and $\pi_{c}$, respectively).  MPT proofs in Ethereum are
generated for 32B-long words; therefore, a domain's public key (which is much
larger than 32B --- usually 256B) requires multiple MPT proofs.  However, these
proofs are highly redundant, and in our scenario, the \name certificate needs
4.11KB to be encoded.  As reported~\cite{VaSz18}, an average size of today's
X.509v3 certificate chain is around 4.75KB; thus, the size of \name
certificates is comparable with TLS certificates deployed currently.
% \medskip


\myparagraph{TLS Clients}
In \name, TLS clients are also blockchain light clients.  That means that
they need to periodically contact the blockchain network, obtain new block
headers (without actual blocks and transactions), and check whether they are
correct.  In Ethereum, block headers are about 508 bytes long; thus, at the time
of writing, the Ethereum main network with 6.75M blocks requires
from \textit{fully light clients}~\cite{light_cli} the storage overhead of about
3.43GB.  However, storing all previous header is not necessary for validating
\name certificates.  TLS clients do not accept \name certificates older than the
\textit{maxStale} parameter. So, if a client rejects certificates that are outdated,
e.g., their storage proofs are older than three days, then the client needs to
keep headers only for three last days (and keep dropping outdated ones), becoming a
\textit{partially light client}~\cite{light_cli}. In this example, the storage
required would be around 10MB. 
% \medskip

\begin{table}[tb]
\begin{center}
    \small
    \begin{tabular}{c|rrrr}
        &\textbf{Min}  &   \textbf{Max}   &   \textbf{Avg.}  &  \textbf{Med.}   \\ \hline
  [\textit{ms}]&6.427 &   11.142 &    7.446 &    7.217 \\
    \end{tabular}
    \caption{The performance of \name certificate validation.}
    \label{tab:valid_perf}
    \end{center}
    \vspace{-0.3cm}
\end{table}
\name clients validate obtained \name certificates (see
\autoref{sec:details:cert_valid}),  what consists of sanity and control
checks, and the validation of storage and code proofs ($\pi_{s}$ and $\pi_{c}$).
(In fact, our client has to validate multiple storage proofs, as Ethereum splits
storage into 32B-long words.)   To evaluate computation overhead, we executed
one hundred \name certificate validations and measured the time required to
execute them.  The obtained performance results are presented in
\autoref{tab:valid_perf}.  As shown, even with our unoptimized implementation,
the average and median values are about 7ms.  % This computational overhead
% introduced is relatively small when compared to network latencies of TLS
% handshakes~\cite{naylor2014cost} and should not be noticed by
% users~\cite{gribble1997system}.  


